The COMICS Tool - Computing Minimal Counterexamples for Discrete-time Markov Chains

This report presents the tool COMICS, which performs model checking and generates counterexamples for DTMCs. For an input DTMC, COMICS computes an abstract system that carries the model checking information and uses this result to compute a critical subsystem, which induces a counterexample. This abstract subsystem can be refined and concretized hierarchically. The tool comes with a command-line version as well as a graphical user interface that allows the user to interactively influence the refinement process of the counterexample.

==> conclusion.tex <==
\medskip
\section{Conclusion and Future Work}
\label{sec:conclusion}

We presented version 1.0 of our tool \toolname which generates
abstract, hierarchically refinable counterexamples for DTMCs. In the
future, we want to integrate the computation of \emph{minimal}
critical subsystems \cite{wimmer-et-al-tacas-2012} and the adaption of
our approaches to \emph{symbolic data structures}. Currently we are
working on an
\emph{incremental version of the Dijkstra algorithm} to improve the
local search and on \emph{compositional counterexamples} to increase the usability of debugging
information, since \prism models are usually built by parallel
composition. 

To speed-up the model checking process,
we will connect our tool to \prism and \mrmc.




==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\emph{Discrete-time Markov chains} (DTMCs) are widely used
to model safety-critical systems with uncertainties. 
Model checking
\emph{probabilistic computation tree logic} (PCTL) \cite{HJ94} properties can be performed by prominent tools like \prism \cite{KNP11} and
\mrmc~\cite{mrmc}. Unfortunately, the implemented numerical methods do not provide diagnostic 
information in form of \emph{counterexamples}, which are very important for debugging and are also needed for CEGAR frameworks \cite{HWZ08}.

Although different approaches were proposed for probabilistic
counterexamples (\cite{AHL05,HKD09,WBB09,jansen-et-al-atva-2011,wimmer-et-al-tacas-2012}),
there is still a lack of efficient and user-friendly \emph{tools}. To fill this gap, we developed the tool
\toolname \iflong(\underline{Co}mputing \underline{Mi}nimal
\underline{C}ounterexample\underline{s})\fi{},
supporting SCC-based model checking~\cite{AJWKB10} and, in case
the property is violated, the \emph{automatic} generation of
\emph{abstract counterexamples}~\cite{jansen-et-al-atva-2011}, which can subsequently be refined either automatically or guided by the user.

While most approaches represent probabilistic counterexamples as sets
of paths, we use (hierarchically abstracted) subgraphs of the input
DTMC, so-called \emph{critical subsystems}.  \iflong This allows for a
much more \emph{compact representation} and a \emph{significant
  decrease in the computational complexity}.  \fi The user can refine
abstract critical subsystems \emph{hierarchically} by choosing
system parts of interest which are to be concretized and further
examined. All computation steps of the hierarchical counterexample
refinement can be \emph{guided and revised}. Though refinement can be
done until a fully concrete counterexample is gained, it seems likely that the
user can gain sufficient debugging information from abstract systems considering
real-world examples with millions of states.
The tool comes with a graphical user interface (GUI) which permits the \emph{visualization and reviewing} of existing test cases and the \emph{creation} of random
examples as well as new test cases.

 The implemented methods result in substantial improvements
regarding the size and the number of computation steps for the
generation of probabilistic counterexamples. The only other available
tool we are aware of is \dipro~\cite{dipro}. However, it does not
support abstract counterexamples, which is crucial for the handling of
large systems. It also does not allow the user to influence the search
process by using his or her expertise. Comparative experiments show that we
can compute reasonably smaller counterexamples in shorter time with
our tool. %Additionally, \toolname comes as a \emph{stand-alone} tool.

In Section~\ref{sec:foundations} we recall some preliminaries regarding DTMCs and counterexamples. In Section~\ref{sec:hierarchical} we give a brief introduction to the
methods implemented in our tool. We describe the features and architecture in Section~\ref{sec:tool} and report on some benchmarks . We conclude the paper in Section~\ref{sec:conclusion}. 
The tool, a detailed manual, and a number of benchmarks are available at the \toolname website\footnote{\url{http://www-i2.informatik.rwth-aachen.de/i2/comics/}}.


==> packages.tex <==
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{tikz} 
% \usepackage[pdfpagelabels=true,linktocpage]{hyperref}
\usepackage{color}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{microtype}
\usepackage{todonotes}
\usepackage{colonequals}
\usepackage{algorithm}
\usepackage{newalg}
\newcounter{oldlinenumber}
% \usepackage{tocbasic}
\usepackage{subfigure}
\usepackage{url}
\usepackage{todonotes}
% \usepackage{appendix}
\usepackage{hyperref}
\usepackage{graphicx}
\usepackage{float}
\usepackage{floatflt} 

\usetikzlibrary{arrows,decorations.pathmorphing,positioning,fit,trees,shapes,shadows} 


==> title.tex <==
\title{The COMICS Tool -- \underline{Co}mputing \underline{Mi}nimal
\underline{C}ounterexample\underline{s} for DTMCs%
\thanks{This work was partly supported by the German Research Council (DFG)
as part of the research project CEBug (AB 461/1-1), the Transregional
Collaborative Research Center AVACS (SFB/TR 14) and the Research Training Group
AlgoSyn (1298) as well as by the Netherlands Organisation for Scientific
Research (NWO) as part of the DFG/NWO Bilateral Research Programme ROCKS.
}}
\author{Nils Jansen\inst{1},
	Erika \'Abrah\'am\inst{1}, Maik Scheffler\inst{1}, 
	Matthias Volk\inst{1}, Andreas Vorpahl\inst{1},
        Ralf Wimmer\inst{2}, Joost-Pieter Katoen\inst{1}, and
        Bernd Becker\inst{2} 
  }

  \institute{RWTH Aachen University, Germany
%   \email{\small{abraham|nils.jansen|katoen}@cs.rwth-aachen.de}
  \and Albert-Ludwigs-University Freiburg, Germany
%   \email{\small{wimmer|becker}@informatik.uni-freiburg.de}
  }

\maketitle

